Robust Membership Encoding: Inference Attacks and Copyright Protection for Deep Learning

Machine learning as a service (MLaaS), and algorithm marketplaces are on a rise. Data holders can easily train complex models on their data using third party provided learning codes. Training accurate ML models requires massive labeled data and advanced learning algorithms. The resulting models are considered as intellectual property of the model owners and their copyright should be protected. Also, MLaaS needs to be trusted not to embed secret information about the training data into the model, such that it could be later retrieved when the model is deployed. In this paper, we present \emph{membership encoding} for training deep neural networks and encoding the membership information, i.e. whether a data point is used for training, for a subset of training data. Membership encoding has several applications in different scenarios, including robust watermarking for model copyright protection, and also the risk analysis of stealthy data embedding privacy attacks. Our encoding algorithm can determine the membership of significantly redacted data points, and is also robust to model compression and fine-tuning. It also enables encoding a significant fraction of the training set, with negligible drop in the model's prediction accuracy.

==> advance.tex <==
\section{Advanced Privacy Attacks with  Membership Encoding}

In this section, we describe some of the advanced privacy attacks using membership encoding: reconstruction attack, a hybrid attack with prior attacks~\cite{song2017machine}.

\paragraphbe{Reconstruction attack.}  The attacker aims at reconstructing a data record which is partially known to him.  The attacker might have some auxiliary information about the data as well.  For example, The adversary might know a DNA sequence with missing sub-sequences, and in addition he knows the candidate sub-sequences.  Adversary can utilize the membership inference attack to perform this reconstruction.  Adversary can query with membership discriminator with all probable combination of the full record. The one which receives highest confidence to be classified as member is the reconstructed record.  Given the high accuracy of our attack, even in the case of missing data, it can be used to perform accurate reconstruction attacks. 

\paragraphbe{Hybrid attack.} Our membership encoding attack can be composed with previous embedding attack to form a stronger attack. Prior work proposed several ways of encoding the exact bits of data record into a ML model while the number of records that can be embedded is limited to a few hundreds for white-box and a dozen records for black-box setting, due to the limited capacity of the model~\cite{song2017machine}. 

In reality, not all bits for a data record are sensitive. Adversary can utilize our membership encoding attack to scale up the embedding attack. For each record that adversary wishes to embed, he splits the record into sensitive attributes and nonsensitive attributes. Adversary then encodes the membership information for these records of interest, using our algorithm, and embeds their sensitive attributes and a compressed version of the nonsensitive attributes (e.g. a short hash) using large data embedding methods~\cite{song2017machine}.  During the decoding (inference) phase, given a redacted input $x^\prime$ with only nonsensitive attributes, adversary first verifies whether  $x^\prime$  is encoded as member.  Our attack is very accurate on partial data.  If it has been a member, the adversary proceeds to compute the compressed version of  $x^\prime$ and finds the corresponding embedded sensitive attributes, using the decoder~\cite{song2017machine}. The major advantage of the hybrid attack is that adversary can use membership encoding to rule out the possible collisions in matching the compressed nonsensitive attribute. In addition, since embedded information for each record is compressed, the model can thus leak information for a large set of records. 


==> figs/prune_plot.tex <==
\begin{figure}[t!]
% \begin{tabular}{c}
\begin{tikzpicture}
\begin{axis}[title style={yshift=-1.5ex}, title=\textbf{VGG white-box},ylabel=Score, xmin=0.1, xmax=0.9, ymin=0., ymax=1, width=0.26\textwidth, grid=both, xlabel=\% pruned params,
name=ax1]
\pgfplotstableread{data/cifar_pruneconv5-1.dat}\mydata;
\addplot[thick, mark=o] table
[x expr=\thisrow{p},y expr=\thisrow{pre}] {\mydata};
% \addlegendentry{encoding precision};
\addplot[thick, mark=triangle] table
[x expr=\thisrow{p},y expr=\thisrow{rec}] {\mydata};
% \addlegendentry{encoding recall};
\addplot[thick, mark=square] table
[x expr=\thisrow{p},y expr=\thisrow{auc}] {\mydata};
% \addlegendentry{encoding AUC};
\addplot[thick, dashed,mark=*] table
[x expr=\thisrow{p},y expr=\thisrow{acc}] {\mydata};
% \addlegendentry{Test accuracy};
\end{axis}

\begin{axis}[title style={yshift=-1.5ex},title=\textbf{VGG white-box  w/ adv},  xlabel=\% pruned params, xmin=0.1, xmax=0.9, ymin=0., ymax=1, legend style = { at = {(0.4,0.02)}, legend columns=2, anchor=south, nodes={scale=0.75, transform shape}},
width=0.26\textwidth, grid=both,
name=ax2, at={(ax1.south east)}, xshift=1cm]
\pgfplotstableread{data/cifar_pruneconv5-1_mal.dat}\mydata;
\addplot[thick, mark=o] table
[x expr=\thisrow{p},y expr=\thisrow{pre}] {\mydata};
% \addlegendentry{encoding precision};
\addplot[thick, mark=triangle] table
[x expr=\thisrow{p},y expr=\thisrow{rec}] {\mydata};
% \addlegendentry{encoding recall};
\addplot[thick, mark=square] table
[x expr=\thisrow{p},y expr=\thisrow{auc}] {\mydata};
% \addlegendentry{encoding AUC};
\addplot[thick, dashed,mark=*] table
[x expr=\thisrow{p},y expr=\thisrow{acc}] {\mydata};
% \addlegendentry{Test accuracy};
\end{axis}
\end{tikzpicture}

\begin{tikzpicture}
\begin{axis}[title style={yshift=-1.5ex},title=\textbf{ResNet}, xlabel=\% pruned parameters, xmin=0.1, xmax=0.9, ymin=0., ymax=1,  ylabel=Score, 
legend style = { at = {(0.4,-0.5)}, legend columns=4, anchor=south},
width=0.26\textwidth, grid=both,
name=ax1]
\pgfplotstableread{data/cifar_pruneres3-2.dat}\mydata;
\addplot[thick, mark=o] table
[x expr=\thisrow{p},y expr=\thisrow{pre}] {\mydata};
% \addlegendentry{Enc pre};
\addplot[thick, mark=triangle] table
[x expr=\thisrow{p},y expr=\thisrow{rec}] {\mydata};
% \addlegendentry{Enc rec};
\addplot[thick, mark=square] table
[x expr=\thisrow{p},y expr=\thisrow{auc}] {\mydata};
% \addlegendentry{Enc AUC};
\addplot[thick, dashed,mark=*] table
[x expr=\thisrow{p},y expr=\thisrow{acc}] {\mydata};
% \addlegendentry{Test acc};
\end{axis}

\begin{axis}[title style={yshift=-1.5ex},title=\textbf{ResNet w/ adv}, xlabel=\% pruned parameters, xmin=0.1, xmax=0.9, ymin=0., ymax=1, legend style = { at = {(0.4,-0.5)}, legend columns=4, anchor=south}, width=0.26\textwidth, grid=both,
name=ax2, at={(ax1.south east)}, xshift=1cm]
\pgfplotstableread{data/cifar_pruneres3-2_mal.dat}\mydata;
\addplot[thick, mark=o] table
[x expr=\thisrow{p},y expr=\thisrow{pre}] {\mydata};
% \addlegendentry{Enc pre};
\addplot[thick, mark=triangle] table
[x expr=\thisrow{p},y expr=\thisrow{rec}] {\mydata};
% \addlegendentry{Enc rec};
\addplot[thick, mark=square] table
[x expr=\thisrow{p},y expr=\thisrow{auc}] {\mydata};
% \addlegendentry{Enc AUC};
\addplot[thick, dashed,mark=*] table
[x expr=\thisrow{p},y expr=\thisrow{acc}] {\mydata};
% \addlegendentry{Test acc};
\end{axis}
\end{tikzpicture}


\begin{tikzpicture}
\begin{axis}[title style={yshift=-1.5ex},title=\textbf{VGG black-box}, xlabel=\% pruned params, ylabel=Score,
xmin=0.1, xmax=0.9, ymin=0., ymax=1, 
width=0.26\textwidth,grid=both,
name=ax1]
\pgfplotstableread{data/cifar_prunefc.dat}\mydata;
\addplot[thick, mark=o] table
[x expr=\thisrow{p},y expr=\thisrow{pre}] {\mydata};
% \addlegendentry{Enc pre};
\addplot[thick, mark=triangle] table
[x expr=\thisrow{p},y expr=\thisrow{rec}] {\mydata};
% \addlegendentry{Enc rec};
\addplot[thick, mark=square] table
[x expr=\thisrow{p},y expr=\thisrow{auc}] {\mydata};
% \addlegendentry{Enc AUC};
\addplot[thick, dashed,mark=*] table
[x expr=\thisrow{p},y expr=\thisrow{acc}] {\mydata};
% \addlegendentry{Test acc};
\end{axis}

\begin{axis}[title style={yshift=-1.5ex},title=\textbf{VGG black-box  w/ adv}, xlabel=\% pruned params, xmin=0.1, xmax=0.9, ymin=0., ymax=1, legend style =  { at = {(-0.2, -0.7)}, legend columns=4, anchor=south},
width=0.26\textwidth, grid=both,
name=ax2, at={(ax1.south east)}, xshift=1cm]
\pgfplotstableread{data/cifar_prunefc_mal.dat}\mydata;
\addplot[thick, mark=o] table
[x expr=\thisrow{p},y expr=\thisrow{pre}] {\mydata};
% \addlegendentry{Enc pre};
\addplot[thick, mark=triangle] table
[x expr=\thisrow{p},y expr=\thisrow{rec}] {\mydata};
% \addlegendentry{Enc rec};
\addplot[thick, mark=square] table
[x expr=\thisrow{p},y expr=\thisrow{auc}] {\mydata};
% \addlegendentry{Enc AUC};
\addplot[thick, dashed,mark=*] table
[x expr=\thisrow{p},y expr=\thisrow{acc}] {\mydata};
% \addlegendentry{Test acc};
\end{axis}

\end{tikzpicture}
\caption{Encoding results on pruned CIFAR10 VGG models.
Plots on the left are the results on models that are pruned naively. 
Plots on the right are the results on models that are adversarially pruned on CIFAR10 for 20 epochs.}
\label{fig:prune}
\end{figure}

